H2-COMPACT: Human-Humanoid Co-Manipulation via Adaptive Contact Trajectory Policies

We present a hierarchical policy-learning framework that enables a legged humanoid to cooperatively carry extended loads with a human partner using only haptic cues for intent inference. At the upper tier, a lightweight behavior-cloning network consumes six-axis force/torque streams from dual wrist-mounted sensors and outputs whole-body planar velocity commands that capture the leader's applied forces. At the lower tier, a deep-reinforcement-learning policy, trained under randomized payloads (0-3 kg) and friction conditions in Isaac Gym and validated in MuJoCo and on a real Unitree G1, maps these high-level twists to stable, under-load joint trajectories. By decoupling intent interpretation (force -> velocity) from legged locomotion (velocity -> joints), our method combines intuitive responsiveness to human inputs with robust, load-adaptive walking. We collect training data without motion-capture or markers, only synchronized RGB video and F/T readings, employing SAM2 and WHAM to extract 3D human pose and velocity. In real-world trials, our humanoid achieves cooperative carry-and-move performance (completion time, trajectory deviation, velocity synchrony, and follower-force) on par with a blindfolded human-follower baseline. This work is the first to demonstrate learned haptic guidance fused with full-body legged control for fluid human-humanoid co-manipulation. Code and videos are available on the H2-COMPACT website.

==> sec/0_abstract.tex <==
\begin{abstract}



\end{abstract}

==> sec/1_intro.tex <==
\section{INTRODUCTION}

Human teams excel at carrying awkward loads by intuitively sensing and responding to each other’s applied forces. Enabling similar fluid collaboration between humans and legged robots remains an open challenge: the robot must both infer the human’s haptic intent and walk stably under the changing load. Prior work in human–robot co‐manipulation has largely focused on fixed‐base manipulators or wheeled platforms, and most legged‐robot controllers either ignore external loads or treat them as disturbances rather than as communication channels (e.g. cite, cite). Meanwhile, state‐of‐the‐art RL policies for legged robots achieve remarkable agility under varying terrains [cite], [cite], but walking under load is still a challenging task for humanoids and also do not integrate haptic feedback to guide motion.

In this paper, we present a two‐policy architecture that unifies haptic‐intent inference with load‐adaptive locomotion on a full‐body humanoid. At the top level, a lightweight neural network takes in  six‐axis forces and torques from dual ATI sensors and outputs a twist—($v_x$, $v_y$, and $\omega_z$)—capturing the human’s intent for direction cues. At the lower level, a Proximal Policy Optimization (PPO)–trained locomotion policy converts these twist commands into joint‐angle trajectories for the Unitree G1, having been trained under randomized payloads (0–3kg) and friction conditions in Isaac Gym and validated in MuJoCo and on hardware [cite], [cite]. By decoupling intent extraction (force→twist) from foothold and posture control (twist→joints), our system achieves both responsive haptic following and robust under‐load walking.

To support cheap, widely deployable data collection, we record only an RGB stream and two F/T sensor channels. We remove background clutter via SAM2 segmentation [cite] and feed the cleaned images into WHAM for 3D human pose and velocity estimation [cite], fusing these kinematics with wrench data for supervised training of the haptic‐inference network. We benchmark against a human–human leader–follower baseline (blindfolded follower), using completion time, trajectory deviation, velocity difference, and average follower force as metrics.

\textbf{Our novel contributions} are: 

%(i) the first demonstration of RL‐based, force‐adaptive humanoid walking during physical co‐manipulation; (ii) a novel haptic‐inference network trained on compact sensor data; (iii) a practical, vision‐only preprocessing pipeline for human kinematics; and (iv) sim‐to‐real validation on a Unitree G1 with quantitative and comparisons to human–human performance.


\begin{enumerate}
    \item  The first demonstration of RL‐based, force‐adaptive humanoid walking during physical co‐manipulation

    \item  A novel haptic‐inference network trained on compact sensor data.

    \item  a practical, vision‐only preprocessing pipeline for human kinematics.

    \item Sim‐to‐real validation on a Unitree G1 with quantitative and comparisons to human–human performance.
\end{enumerate}


==> sec/2_relatedwork.tex <==

\section{Related Works}
\label{sec:related}

\subsection{Physical Human–Robot Co-Manipulation}

Physical human–robot collaboration for co–manipulation has been studied extensively on fixed‐base manipulators and wheeled platforms. Early work employed variable‐impedance control to let a robot comply with human force inputs \cite{ikeura1995variable, duchaine2007general}, while subsequent approaches used state machines or probabilistic models to disambiguate translation versus rotation during bi‐manual carrying tasks \cite{karayiannidis2014mapping, thobbi2011using}. Human–human dyad experiments have revealed that interaction forces are not minimized but convey intent, and that lateral and rotational motions follow minimum–jerk–like profiles even under blindfolded conditions \cite{mielke2020analysis}. Bi‐manual co–manipulation on humanoid platforms remains rare: Bussy \emph{et al.} demonstrated haptic joint transportation on a Baxter robot \cite{bussy2012proactive}, and more recent studies have integrated EMG or motion‐capture cues to enhance compliance \cite{peternel2017human, rozo2016learning}. However, these methods either assume known trajectories or rely on low‐dimensional manipulators, and none yet combine full‐body legged locomotion with haptic guidance.



\subsection{Reinforcement Learning for Force-Adaptive Humanoid Locomotion}

Reinforcement learning (RL) has been successfully applied to achieve stable locomotion in quadrupeds \cite{Hwangbo_2019,Lee_2020,tan2018simtoreallearningagilelocomotion} and in humanoids \cite{gu2024humanoidgymreinforcementlearninghumanoid,Singh_2024,wang2025beamdojolearningagilehumanoid}. Compared to classical optimal-control-problem (OCP) based controllers, which must solve high-dimensional trajectory optimizations online—inducing significant latency and exhibiting sensitivity to modeling errors \cite{doi:10.1177/027836498400300206,10286076}—RL-trained policies learn end-to-end control mappings offline and execute in constant time via a single network inference \cite{schulman2017proximalpolicyoptimizationalgorithms,pmlr-v80-haarnoja18b}. 

The task defined in our paper requires forceful interaction with the human when performing co-manipulation and carrying load while walking. Some of the previous work has learned a policy for tasks requiring forceful interactions, such as dribbling a ball in both quadrupeds \cite{ji2023dribblebotdynamicleggedmanipulation} and humanoids \cite{Haarnoja_2024}, door-opening \cite{zhang2024learningopentraversedoors} and learning control force or compliance at the end effector of quadrupeds with an mounted arm \cite{portela2024learningforcecontrollegged}. \textcolor{red}{to add some humanoid papers here}

==> sec/3_method.tex <==
\section{Methodology}
\label{sec:methodology}

\subsection{System Overview}
\textcolor{red}{HERE WE NEED TO ADD A whole system overview diagram }

\subsubsection{Control Architecture}

Our co–manipulation controller is organized as a cascade of two learned policies, each optimized for a distinct aspect of the physical interaction. At the highest level, a lightweight neural policy ingests the six–axis readings from the two ATI force/torque sensors mounted on the handles and directly outputs a desired planar twist—linear velocities $(v_x,v_y)$ and yaw rate $\omega_z$—that reflects the human’s haptic intent. This haptic–inference network is trained offline on human–human demonstration data to reproduce the subtle force cues that guide a natural carrying motion.

These high–level velocity commands then serve as reference inputs to a second policy, which is trained via deep reinforcement learning to convert twists into precise joint–angle trajectories for the Unitree G1. During training, this locomotion policy experiences a variety of payloads (0–3kg) and friction conditions, and learns to maintain balance and faithfully track arbitrary planar twists under load. By separating intent inference (force–to–velocity) from foothold and posture control (velocity–to–joints), our two–policy architecture achieves both intuitive responsiveness to human guidance and robust, under–load walking stability.  


\subsection{}

\subsection{RL-Based Load-Adaptive Locomotion}
\subsubsection{Problem Formulation}
%Include the formal RL mathematical definitions (state vector, action vector, reward function, and PPO formula).
We formulate our load-adaptive locomotion task as a POMDP and utilize Proximal Policy Optimization (PPO) \cite{schulman2017proximalpolicyoptimizationalgorithms} to learn a parameterized policy \(\pi_\theta(a_t \mid o_{ t})\) that maximizes the expected discounted return while ensuring stable and force-aligned locomotion. We implement PPO from the RSL-RL library \cite{rudin2022learning} with both actor and critic as three‐layer MLPs. 
Mathematically,
\[
\mathcal{M} = \bigl(\,\mathcal{S},\;\mathcal{A},\;T,\;\mathcal{O},\;R,\;\gamma\bigr),
\] 
where a full simulator state \(\mathbf{s}_t\in\mathcal S\) evolves via
\(T(\mathbf{s}_{t+1}\mid\mathbf{s}_t,\mathbf{a}_t)\), but at deployment
the agent only receives observation \(\mathbf{o}_t\in\mathcal O\). $R$ is the scalar reward function per step, and $\gamma\in[0,1]$ is the discount factor balancing immediate versus long‐term returns. 
We parameterize a feed-forward policy
\(\pi_\theta(a_t\mid o_t)\) and train it with PPO to maximize
\(\displaystyle J(\theta)=\mathbb{E}_{\pi_\theta}\bigl[\sum_t\gamma^t\,r_t\bigr]\).
To stabilize updates we use the clipped surrogate
\[
\mathcal{L}_{\pi}(\theta)
= \mathbb{E}_t\Bigl[\min\bigl(\rho_t\,\widehat A_t,\,
\mathrm{clip}(\rho_t,1-\epsilon,1+\epsilon)\,\widehat A_t\bigr)\Bigr],
\]
,where
\[
\rho_{t}
= \frac{\pi_{\theta}(a_{t}\mid o_{t})}
       {\pi_{\theta_{\text{old}}}(a_{t}\mid o_{t})}
\]
is the likelihood ratio, \(\epsilon>0\) is the PPO clipping parameter that bounds how far the new policy is allowed to deviate from the old one in each update, and \(\widehat A_{t}\) is an estimate of the advantage function:
\[
\widehat A_{t}
= {\sum_{l=0}^{T-t}\gamma^{\,l}r_{t+l}}
- V_{\phi}(o_{t}),
\]
with \(V_{\phi}(o_{t})\) the value‐function baseline.  




\subsubsection{Training for Load-Adaptation}
Building on Unitree’s official RL framework, which follows \cite{gu2024humanoidgymreinforcementlearninghumanoid} by using an asymmetric actor‐critic for lower‐body control and phase‐based rewards to learn periodic gaits, we train our policy to handle dynamic payloads by applying randomized external forces at the wrist‐roll link on both hands within Isaac Gym \cite{makoviychuk2021isaacgymhighperformance}. During each episode, each wrist links receive a force in the z-direction sampled from
\[
f \sim \mathcal{U}([-F_{\max},\,F_{\max}]),
\]
emulating variable load mass and distribution. We set \(F_{\max}=15\) N to match the robot’s nominal payload capacity, and choose a lower bound of \(-3\) N to allow for small assisting (upward) forces that a human partner might exert when lifting. This randomized force perturbation ensures the learned policy dynamically compensates for both resisting and assisting loads during co‐manipulation.


At each timestep \(t\), the observation vector is
\[
O_t = \bigl[\,
\omega_t,\;
\hat{g_t},\;
C_t,\;
(q_t - q_{0,t}),\;
\dot q_t,\;
a_{t-1},\;
\sin(2\pi \phi_t),\;
\cos(2\pi \phi_t)
\bigr],
\]
where \(\omega_t\) is the body’s angular velocity, \(g_t\) the projected gravity vector, \(C_t\) the three command values for linear velocity in x and y direction and angular velocity in the z direction, \(q_t\) and \(\dot q_t\) the 12-DOF joint positions and velocities for legs, \(q_{o,t}\) the default joint positions, and \(\phi_t\) the normalized gait phase. The network then outputs desired legs joint positions \(a_t\), which are converted to torques by
\[
\tau_{t,i} = K_{p,i}\,(a_{t,i} - a_{0,t,i}) \;-\; K_{d,i}\,\dot a_{t,i},
\]
where \(i\) indexes each joint. 

Further implementation details of training parameters and reward functions are in Appendix \ref{tab:hyperparameters} and Appendix \ref{tab:rewards_refined} respectively.


\subsubsection{Simulation-to-Real Considerations}
We leverage Isaac Gym for high-speed, GPU-based parallel training of our RL policy and conduct sim2sim validation in MuJoCo \cite{todorov2012mujoco}, which is known for its accurate physical dynamics \cite{gu2024humanoidgymreinforcementlearninghumanoid}. This workflow combines the rapid experimentation of Isaac Gym with the high-fidelity but slower CPU-based MuJoCo environment. Finally, the trained policy is deployed and evaluated in sim2real transfer experiments on the physical Unitree G1-23 DOF robot.

To increase robustness to real-world variability, we apply domain randomization throughout training. Specifically, at the start of each episode we randomly perturb the ground contact properties, the robot’s base mass, and apply external pushes, as summarized in Appendix \ref{tab:domain_rand}. These randomizations follows the principles of \cite{tobin2017domainrandomizationtransferringdeep} and helps prevent overfitting to any single simulation configuration, resulting a policy that remains stable under variations in surface friction, load, and unexpected collisions in both sim-to-sim and sim-to-real transfer.

\subsection{Data Preprocessing}

All sensor streams—force and torque from the two ATI Mini45 units and RGB video—are time‐stamped in ROS and aligned in post‐processing to ensure perfect synchronization.  This unified timeline allows us to associate each image frame with the corresponding six‐axis wrench readings on both handles.

\paragraph{Image Cleaning via SAM2}  
To make pose estimation robust in cluttered or crowded scenes, we first apply the Segment Anything Model v2 (SAM2) \cite{ravi2024sam2segmentimages} to each RGB frame.  SAM2 produces binary masks for all non‐human objects and extraneous persons.  We then inpaint these masked regions by copying the original background texture, effectively “erasing’’ occluders while preserving the true scene context.  This preprocessing step ensures that downstream pose estimators operate on clean, human‐only imagery, even in busy environments.

\paragraph{3D Pose and Velocity Extraction with WHAM}  
Cleaned frames are passed to the WHAM 3D human pose‐and‐velocity network \cite{shin2024whamreconstructingworldgroundedhumans}, which outputs joint positions in a metric world frame at each timestamp.  We compute linear and angular velocities by finite‐difference of the wrist and torso joints over consecutive frames: \textcolor{red}{@hao add the relevent method you used for velocity tracking}
\[
  v_h(t) \;=\; \frac{p_h(t) - p_h(t - \Delta t)}{\Delta t}
  \quad,\quad
  \omega_h(t) \;=\; \frac{\theta_h(t) - \theta_h(t - \Delta t)}{\Delta t}\,.
\]
Here \(p_h\) and \(\theta_h\) denote the 3D position and orientation of the human’s grasping pose, and \(\Delta t\) is the frame interval.

\paragraph{Fusion for Model Training}  
Finally, we pair each \( \{v_h(t),\omega_h(t)\}\) sample with the synchronized six‐axis force/torque readings from both handles, yielding a compact, sensor‐agnostic dataset.  This fusion of haptic and kinematic streams forms the basis for training our co‐manipulation intent model, without any specialized motion‐capture hardware.  




==> sec/4_experiments.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{Hardware Design}

We modified a box for data-collection by adding 3D-printed handles to mount an ATI Mini45 six-axis force/torque sensor via a bespoke adapter (Fig.~\ref{hardware_box}). The sensor was interfaced through an EtherCAT OEM F/T module \cite{ati2024mini45} and powered by a 24 V LiPo battery. Force/torque signals were sampled at 1 kHz and streamed over USB into a laptop running ROS, where they were time synchronized with image data and recorded into rosbag \cite{inproceedings}.

For on-robot deployment (Fig.~\ref{hardware_robot}), the ATI Mini45 was affixed to the Unitree G1 wrist using custom 3D-printed mounts. It drew power from the robot’s internal 24V bus, and all sensor data were transmitted via EtherCAT to the onboard computer \cite{unitree2025g1developer}. 




% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{figs/hardware_box.png}
%   \caption{Hardware box.}
%   \label{hardware_box}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{figs/unitree_g1.jpg}
%   \caption{Unitree G1 robot.}
%   \label{hardware_robot}
% \end{figure}

\subsection{Data Collection}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figs/data_collection.drawio.png}
%     \caption{Data collection.}
%     \label{data_collection}
% \end{figure}

\begin{figure*}[t]
  \centering
    \centering
    \includegraphics[width=\textwidth]{figs/data_robot.png}
    \caption{data robots}
    \label{data_robot}
\end{figure*}


\begin{figure*}[t]
  \centering
    \centering
    \includegraphics[width=\textwidth]{figs/data_collection.png}
    \caption{data setup}
    \label{data_setup}
\end{figure*}


We collect data in dyadic leader–follower trials using the hardware shown in Fig.~\ref{data_collection}. The leader and the follower each grasped one handle of the instrumented box, with an ATI Mini45 six‐axis F/T sensor mounted on the follower’s side. The follower carried a computation backpack containing a battery and onboard computer, which streamed force/torque readings at 1 kHz over EtherCAT into ROS. A static RGB camera recorded the entire interaction. All sensor and video streams were time-synchronized and recorded with rosbag.

We defined eight primitive motions (Fig.~\ref{data_setup}): forward, backward, left, right translations; leader-centric clockwise and anti-clockwise rotations; and follower-centric clockwise and anti-clockwise rotations. Each primitive was executed in three trials under four payload conditions, yielding 96 total trajectories. To enforce pure haptic guidance, the follower was blindfolded and had no prior knowledge of the intended motion or trajectory, relying solely on haptic cues to interpret and follow the leader's input.


add image of 
i. over force and torque arrows over the data collection image with wham mesh after sam2 mask removal

\subsection{Real world testing with Humanoid robot}
Using unitree G1
\begin{figure*}[t]
  \centering
    \centering
    \includegraphics[width=\textwidth]{figs/comanipulation_.pdf}
    \caption{co-manipulation}
    \label{robot_comanipulation}
\end{figure*}
i. image with human and humanoid holding box,
ii. time series image of co-manipulation.

% \subsubsection{Evaluation metrics}

% To rigorously evaluate human–humanoid co-manipulation, we employ four complementary metrics, inspired by prior co-manipulation studies (cite the two papers here)

% \paragraph{Completion Time}  
% We denote by $T_c$ the elapsed time from the onset of cooperative motion ($t_s$) to task completion ($t_e$). We detect $t_s$ when the object’s centre of mass first moves beyond 5\% of the total displacement, and $t_e$ when it remains within 95\% of the goal for at least 0.5s. Formally,
% \begin{equation}
%   T_c \;=\; t_e - t_s
%   \label{eq:completion_time}
% \end{equation}
% \emph{What it is:} The total carry-and-move duration.  
% \emph{Why it matters:} If $T_c$ is much larger than a natural human pace, the robot may be impeding rather than assisting.

% \paragraph{Mean Trajectory Deviation}  
% We quantify spatial agreement by averaging the Euclidean distance between human and robot end-effector positions:
% \begin{equation}
%   \Delta_{\rm traj}
%   = \frac{1}{t_e - t_s}
%     \int_{t_s}^{t_e}
%     \bigl\|x_h(t) - x_r(t)\bigr\| \,\mathrm{d}t
%   \label{eq:traj_dev}
% \end{equation}
% where $x_h(t),x_r(t)\in\mathbb{R}^3$ are the human and robot trajectories.  
% \emph{What it is:} The average hand-path mismatch.  
% \emph{Why it matters:} A low $\Delta_{\rm traj}$ indicates the robot is moving intuitively alongside the human; large values reveal mis-coordination.

% \paragraph{Mean Velocity Difference}  
% We measure kinematic synchrony by the average speed mismatch:
% \begin{equation}
%   \Delta_{v}
%   = \frac{1}{t_e - t_s}
%     \int_{t_s}^{t_e}
%     \bigl\|\dot x_h(t) - \dot x_r(t)\bigr\| \,\mathrm{d}t
%   \label{eq:vel_diff}
% \end{equation}
% with $\dot x_h,\dot x_r\in\mathbb{R}^3$ denoting instantaneous velocities.  
% \emph{What it is:} The mean absolute difference in speed.  
% \emph{Why it matters:} Even if positions align, jerky or lagging velocity profiles are uncomfortable and signal poor coupling.

% \paragraph{Speed Constraint}  
% Because the Unitree G1’s maximum walking speed is 0.8m/s, human followers were instructed to cap their peak walking velocity at this value.  
% This ensures that completion time and deviation metrics (Eqs.~\eqref{eq:completion_time}–\eqref{eq:vel_diff}) reflect cooperative performance, not a human sprint outpacing the robot.

% For performing these evaluations, we used vicon motion capture system with the  specially design marker mount [cite] we compare our results with the human human dyad pair, with ne leader and one follower and follower is blind folded and we performed 10 trails with 2 pairs for transporting the cardboard box with varying load, 

\subsubsection{Evaluation metrics}

To rigorously evaluate human–humanoid co-manipulation, we employ four complementary metrics, inspired by prior co-manipulation studies \cite{mielke2020analysis, sirintuna2022adaptive}.

\paragraph{Completion Time}  
We denote by $T_c$ the elapsed time from the onset of cooperative motion ($t_s$) to task completion ($t_e$). We detect $t_s$ when the object’s centre of mass first moves beyond 5\% of the total displacement, and $t_e$ when it remains within 95\% of the goal for at least 0.5s. Formally,
\[
  T_c = t_e - t_s
  \label{eq:completion_time}
\]
\emph{What it is:} The total carry-and-move duration.  
\emph{Why it matters:} If $T_c$ exceeds typical human–human times, the robot may be hindering dexterity rather than assisting.

\paragraph{Mean Trajectory Deviation}  
We quantify spatial agreement by averaging the Euclidean distance between human and robot end-effector positions:
\[
  \Delta_{\rm traj}
  = \frac{1}{t_e - t_s}
    \int_{t_s}^{t_e}
    \bigl\|x_h(t) - x_r(t)\bigr\| \,\mathrm{d}t
  \label{eq:traj_dev}
\]
where $x_h(t),x_r(t)\in\mathbb{R}^3$ are the human and robot trajectories.  
\emph{What it is:} The average hand-path mismatch.  
\emph{Why it matters:} A low $\Delta_{\rm traj}$ indicates the robot is moving intuitively alongside the human; large values reveal mis-coordination.

\paragraph{Mean Velocity Difference}  
We measure kinematic synchrony by the average speed mismatch:
\[
  \Delta_{v}
  = \frac{1}{t_e - t_s}
    \int_{t_s}^{t_e}
    \bigl\|\dot x_h(t) - \dot x_r(t)\bigr\| \,\mathrm{d}t
  \label{eq:vel_diff}
\]
with $\dot x_h,\dot x_r\in\mathbb{R}^3$ denoting instantaneous velocities.  
\emph{What it is:} The mean absolute difference in speed.  
\emph{Why it matters:} Even if positions align, jerky or lagging velocity profiles are uncomfortable and signal poor coupling.

\paragraph{Average Follower Force}  
We define the mean follower force $\bar F$ as
\[
  \bar F
  = \frac{1}{t_e - t_s}
    \int_{t_s}^{t_e}
    \bigl(\|f_1(t)\| + \|f_2(t)\|\bigr)\,\mathrm{d}t
  \label{eq:force}
\]
where $f_1(t),f_2(t)\in\mathbb{R}^3$ are the instantaneous force vectors measured by the two ATI sensors.  
\emph{What it is:} The average total magnitude of force the follower (human or robot) senses from the leader’s haptic inputs.  
\emph{Why it matters:} A lower $\bar F$ indicates the follower is highly responsive—interpreting the leader’s intent and moving with minimal force—while high values imply the leader must push harder to drive cooperation.  



All kinematic data were recorded with a Vicon motion capture system and a custom 3D-printed marker mount \cite{10977589}.  We benchmark human–humanoid performance against a human–human baseline collected using three dyads (one leader, one blindfolded follower) each performing ten trials of box transport under varying load conditions \cite{mielke2020analysis}.  




==> sec/5_results.tex <==
\section{Result}
\label{sec:result}

\begin{figure}[]
  \includegraphics[width=\columnwidth]{figs/position_traj.eps}
 \caption{Position tracking of the humanoid and human followers relative to the leader in both scenarios, along with the corresponding position error between the leader and each follower. \textbf{Top:} Motion along the x-axis. \textbf{Bottom:} Motion along the y-axis.}
  \label{fig:position}
\end{figure}

\begin{figure}[]
  \includegraphics[width=\columnwidth]{figs/vel_traj.eps}
    \caption{Velocity error tracking between the leader and the corresponding humanoid or human follower in each case. \textbf{Top:} Tracking along the x-axis. \textbf{Bottom:} Tracking along the y-axis.}
  \label{fig:velocity}
\end{figure}

\begin{table}[t]
  \centering
  \caption{Comparison of evaluation metrics between human–human and human–humanoid co–manipulation (mean\,$\pm$\,std).}
  \label{tab:metrics_comparison}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Metric} & \textbf{Human–Human} & \textbf{Human–Humanoid} \\
    \midrule
    Completion Time $T_c$ (s) $\downarrow$  
      & 23.78  
      & 51.47 \\

    Trajectory Deviation $\Delta_{\rm traj}$ (m) $\downarrow$  
      & 0.1109  
      & 0.1294 \\

    Velocity Difference $\Delta_v$ (m/s) $\downarrow$  
      & 0.165  
      & 0.143 \\

    Average Follower Force $\bar F$ (N) $\downarrow$ 
      & 17.355 
      & 16.230 \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Load-Adaptive RL policy}

\begin{figure}[h!]
  \centering
  \includegraphics[width=\columnwidth]{figs/rl_done.pdf}
  \caption{Sim2Sim transfer of the baseline and load‐adaptive policies in MuJoCo under a constant 30\,N payload. \textbf{Top:} The baseline policy tips and falls (left) whereas the load‐adaptive policy holds the box stably (right). \textbf{Bottom:} Commanded vs.\ actual base x‐velocity, y‐velocity, and yaw angular velocity rate over 0–10\,s for both controllers (red dotted: baseline; green solid: load‐adaptive), showcasing the adaptive policy’s smooth, accurate tracking under load.}
  \label{fig:sim2sim_transfer}
\end{figure}



We tested the policy as a sim2sim transfer to the MuJoCo simulator and compared the base linear velocities (along both x- and y-axes) and yaw rate to verify the training under our use cases.
In every trial the robot carried a constant 30 N payload. The plots shows the commanded versus actual x-velocity (first) and y-velocity (second), and the bottom row shows the yaw rate for both the baseline policy (labeled red) and our load-adaptive policy (labeled green).

Under the applied load, the baseline controller exhibits large overshoots, oscillations, and even reversals in both linear channels—behavior that ultimately leads to instability (as seen in the fallen pose on the left of first row). By contrast, the load-adaptive policy tracks the constant command almost perfectly across all three channels, with minimal transient error and smooth convergence to the target velocity, demonstrating substantially improved stability and payload robustness in sim2sim transfer. 

\subsection{Ablation study}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figs/RL_overview_.pdf}
  \caption{Overview of our training and deployment pipeline. 
    (\textbf{a}) Visualization of training on IsaacGym: green arrows denote the magnitude of forces applied to the wrists. 
    (\textbf{b}) Successful sim-to-sim transfer of the walking policy in MuJoCo. 
    (\textbf{c}) Real-world deployment of our trained policy for human–humanoid co-manipulation.}
  \label{fig:rl_overview}
\end{figure*}



==> sec/6_conclusion.tex <==
\section{CONCLUSION}
